Approximation Algorithms for Fair Range Clustering

This paper studies the fair range clustering problem in which the data points are from different demographic groups and the goal is to pick $k$ centers with the minimum clustering cost such that each group is at least minimally represented in the centers set and no group dominates the centers set. More precisely, given a set of $n$ points in a metric space $(P,d)$ where each point belongs to one of the $\ell$ different demographics (i.e., $P = P_1 \uplus P_2 \uplus \cdots \uplus P_\ell$) and a set of $\ell$ intervals $[\alpha_1, \beta_1], \cdots, [\alpha_\ell, \beta_\ell]$ on desired number of centers from each group, the goal is to pick a set of $k$ centers $C$ with minimum $\ell_p$-clustering cost (i.e., $(\sum_{v\in P} d(v,C)^p)^{1/p}$) such that for each group $i\in \ell$, $|C\cap P_i| \in [\alpha_i, \beta_i]$. In particular, the fair range $\ell_p$-clustering captures fair range $k$-center, $k$-median and $k$-means as its special cases. In this work, we provide efficient constant factor approximation algorithms for fair range $\ell_p$-clustering for all values of $p\in [1,\infty)$.

==> notations.tex <==
\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}[section]

\newtheorem{result}{Result}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim} 
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{question}[theorem]{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{definition}[theorem]{Definition}


\theoremstyle{plain}%
\theoremheaderfont{\bf} \theorembodyfont{\upshape}%
\newtheorem{remark}[theorem]{Remark}%
\newtheorem*{remark:unnumbered}[theorem]{Remark}%
\newtheorem*{remarks}[theorem]{Remarks}%
\newtheorem{defn}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise_h}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}%

% Proof environment

\theoremheaderfont{\em}%
\theorembodyfont{\upshape}%
\theoremstyle{nonumberplain}%
\theoremseparator{}%
\theoremsymbol{\myqedsymbol}%
\newtheorem{proof}{Proof:}%

\newcommand{\myqedsymbol}{$\square$}

\newtheorem{proofof}{Proof of\!}%



\newcommand{\eps}{\varepsilon}%
\def\bar{\overline}
\def\floor#1{\lfloor {#1} \rfloor}
\def\ceil#1{\lceil {#1} \rceil}
\def\script#1{\mathcal{#1}}
\def\etal{\text{et al.}\xspace}
\def\Union{\bigcup}
\def\sep{\;|\;}
\def\card#1{|#1|}
\def\set#1{\{#1\}}
\def\E{\mathbf{E}}
\def\Var{\mathbf{Var}}

%\def\arc#1{\accentset{\rightharpoonup}{#1}}

\newcommand{\argmax}{\mathrm{argmax}{}\xspace}
\newcommand{\argmin}{\mathrm{argmin}{}\xspace}

\def\wrt{\text{w.r.t.}\xspace}

\newcommand{\polylog}{\mathop{\mathrm{polylog}}}%
\newcommand{\poly}{\mathop{\mathrm{poly}}}%

\def\whp{\text{w.h.p.}}
\newcommand{\tldO}{\widetilde{O}}%
\newcommand{\tldOmega}{\widetilde{\Omega}}%
\newcommand{\tldTheta}{\widetilde{\Theta}}%


\def\sA{\script{A}}
\def\sB{\script{B}}
\def\sC{\script{C}}
\def\sD{\script{D}}
\def\sE{\script{E}}
\def\sF{\script{F}}
\def\sG{\script{G}}
\def\sI{\script{I}}
\def\sL{\script{L}}
\def\sK{\script{K}}
\def\sM{\script{M}}
\def\sN{\script{N}}
\def\sO{\script{O}}
\def\sP{\script{P}}
\def\sQ{\script{Q}}
\def\sR{\script{R}}
\def\sS{\script{S}}
\def\sT{\script{T}}
\def\sU{\script{U}}
\def\sV{\script{V}}
\def\sX{\script{X}}
\def\sY{\script{Y}}
\def\sW{\script{W}}
\def\sZ{\script{Z}}


\def\NP{\ensuremath{\mathrm{\mathbf{NP}}}}
%\def\cost{\mathrm{cost}}
\def\dist{\mathrm{dist}}
\def\lp{\script{LP}}
%\def\nn{\mathrm{NN}}
\def\scllp{\textsc{SimplifiedLP}}
\def\cllp{\textsc{FairRangeLP}}
\def\clla{\textsc{FacilityMatAlg}}
\def\cllc{\textsc{CenterPartAlg}}
\def\optcllp{BasicClusterLP}
%\def\spcllp{SparseClusterLP}
\def\opt{\textsc{OPT}}
\def\rem{\mathrm{rem}}
\def\kcenter{k\mathrm{center}}

%\def\clcp{ClusterCP}
%\def\optclcp{BasicClusterCP}

\newcommand\faircost{{\operatorname{fair-cost}}}
\newcommand\cost{{\operatorname{cost}}}
\newcommand\vol{{\operatorname{vol}}}
\def\R{\script{R}}
\newcommand{\sol}{\textsc{SOL}}%
\def\Y{\boldsymbol{Y}}
\def\X{\boldsymbol{X}}
\def\g{{\boldsymbol{g}}}
\def\solsp{\mathcal{P}}
\def\intSolSp{\mathcal{Q}}

\def\nn{\textsf{NN}}
\def\inc{\boldsymbol{inc}}
\def\slack{\boldsymbol{slack}}
\def\excess{\boldsymbol{f}}
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\FacMat{\textsc{FacilityMatroid}}
\def\FairClust{\textsc{FairKClustering}}

\newcommand\ali[1]{\textcolor{red}{AV: #1}}

